Dark Matter detection via lepton cosmic rays

Recent observations of lepton cosmic rays, coming from the PAMELA and FERMI experiments, have pushed our understanding of the interstellar medium and cosmic rays sources to unprecedented levels. The imprint of dark matter on lepton cosmic rays is the most exciting explanation of both PAMELA's positron excess and FERMI's total flux of electrons. Alternatively, supernovae are astrophysical objects with the same potential to explain these observations. In this work, we present an updated study of the astrophysical sources of lepton cosmic rays and the possible trace of a dark matter signal on the positron excess and total flux of electrons.

==> tex/newcommands.tex <==
%\newcommand{cmd}[args][opt]{def} 
%\renewcommand{\arraystretch}{1.1} 

% \newcommand{\ie}{{\it i.e. }}
% \newcommand{\roots}{{\sqrt{s}}}
% 
% \newcommand{\lD}{\lambda_{\tn{D}}}
% 
% \newcommand{\tpow}[1]{\times 10^{#1}} % 10^{x}
% \newcommand{\mass}[1]{ m_{#1} }
% \newcommand{\ener}[1]{ \varepsilon_{#1} } 
% \newcommand{\kin}[1]{ \tn{T}_{#1} }
% \newcommand{\mom}[1]{ p_{#1} }
% \newcommand{\momv}[1]{ \vec{p}_{#1}}
% \newcommand{\dnde}[1]{\frac{dn}{d\ener{#1}}}
% \newcommand{\curr}[1]{ \mathcal{J}_{#1} }
% 
% % particles
% \newcommand{\nue}{\nu_{e}}
% \newcommand{\nuebar}{\bar{\nu}_{e}}
% \newcommand{\numu}{\nu_{\mu}}
% \newcommand{\numubar}{\bar{\nu}_{\mu}}
% \newcommand{\nutau}{\nu_{\tau}}
% \newcommand{\nutaubar}{\bar{\nu}_{\tau}}
% 
% \newcommand{\fref}[1]{{\small\textnormal{\ref{#1}}}}
% \newcommand{\citeeq}[1]{{\small\textnormal{Equation}}~\fref{#1}}
% \newcommand{\citeeqq}[2]{{\small\textnormal{Equations}}~\ref{#1} and \fref{#2}}
% \newcommand{\citefig}[1]{{\small\textnormal{Figure}}~\fref{#1}}
% \newcommand{\citefigg}[2]{{\small\textnormal{Figure}}~\fref{#1} and \fref{#2}}
% \newcommand{\citetab}[1]{{\small\textnormal{Table}}~\fref{#1}}
% \newcommand{\citecha}[1]{{\small\textnormal{Chapter}}~\fref{#1}}
% \newcommand{\citeapp}[1]{{\small\textnormal{Appendix}}~\fref{#1}}
% \newcommand{\citesec}[1]{{\small\textnormal{Section}}~\fref{#1}}
% \newcommand{\citeref}[1]{{\small\textnormal{Reference}}~\cite{#1}}


\newenvironment{fig}{\begin{figure}[tp]\vspace{0ex}\begin{minipage}{\textwidth}\centering}{\end{minipage}\end{figure}}
\newenvironment{tab}{\begin{table}[tp]\vspace{0ex}\begin{minipage}{\textwidth}\centering}{\end{minipage} \end{table}}
\newenvironment{prechap}{\begin{center}\begin{minipage}{0.85\textwidth}}{\end{minipage}\end{center}}
\newenvironment{eq}{\begin{eqnarray}}{\end{eqnarray}}


% New definition of square root:
% it renames \sqrt as \oldsqrt
\let\oldsqrt\sqrt
% it defines the new \sqrt in terms of the old one
\def\sqrt{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\oldsqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.2\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}

